PhaseCode: Fast and Efficient Compressive Phase Retrieval based on Sparse-Graph-Codes

We consider the problem of recovering a $K$-sparse complex signal $x$ from $m$ intensity measurements. We propose the PhaseCode algorithm, and show that in the noiseless case, PhaseCode can recover an arbitrarily-close-to-one fraction of the $K$ non-zero signal components using only slightly more than $4K$ measurements when the support of the signal is uniformly random, with order-optimal time and memory complexity of $\Theta(K)$. It is known that the fundamental limit for the number of measurements in compressive phase retrieval problem is $4K - o(K)$ to recover the signal exactly and with no assumptions on its support distribution. This shows that under mild relaxation of the conditions, our algorithm is the first constructive \emph{capacity-approaching} compressive phase retrieval algorithm: in fact, our algorithm is also order-optimal in complexity and memory. Next, motivated by some important practical classes of optical systems, we consider a Fourier-friendly constrained measurement setting, and show that its performance matches that of the unconstrained setting. In the Fourier-friendly setting that we consider, the measurement matrix is constrained to be a cascade of Fourier matrices and diagonal matrices. We further demonstrate how PhaseCode can be robustified to noise. Throughout, we provide extensive simulation results that validate the practical power of our proposed algorithms for the sparse unconstrained and Fourier-friendly measurement settings, for noiseless and noisy scenarios. A key contribution of our work is the novel use of coding-theoretic tools like density evolution methods for the design and analysis of fast and efficient algorithms for compressive phase-retrieval problems.

==> ref.tex <==

\begin{thebibliography}{X}

\bibitem{Bollobas} B.~Bollobas, ``Random graphs,'' \emph{Cambridge University Press}, 2001.

\bibitem{Jaggi} S.~Cai, M.~Bakshi, S.~Jaggi, and M.~Chen, ``SUPER: Sparse signals with Unknown Phases Efficiently Recovered,'' \emph{arXiv preprint arXiv:1401.4451}, 2014.

\bibitem{fanny} V.~Pohl, F.~Yang, and H.~Boche, ``Phase retrieval from low rate samples,'' \emph{arXiv preprint arXiv:1311.7045}, 2013.

\bibitem{Balan} R.~Balan, P.~G.~Casazza, and D.~Edidin, ``On signal reconstruction without phase,'' \emph{Applied and Computational Harmonic Analysis}, vol.~20, no.~3, May 2009.

\bibitem{RU01} T.~Richardson and R.~Urbanke, ``The Capacity of Low-Density Parity-Check Codes Under Message-Passing Decoding'' \emph{IEEE Transactions on Information
Theory}, vol. 47, pp. 599--618, Feb. 2001.

\bibitem{Sameer} S.~Pawar and K.~Ramchandran, ``Computing a $k$-sparse $n$-length Discrete Fourier Transform using at most $4k$ samples and $O(k \log k)$ complexity,'' \emph{arXiv preprint arXiv:1305.0870}, 2013.

\bibitem{Bandeira} A.~S.~Bandeira, J.~Cahill, D.~G.~Mixon, and A.~A.~Nelson, ``Fundamental Limits of Phase Retrieval,''
\emph{Proc. 10th Intern. Conf. on Sampling Theory and Applications (SampTA)}, July 2013.

\bibitem{Milane} R.~P.~Milane, ``Phase retrieval in crystallography and optics,'' \emph{J. Opt. Soc. Am. A}, vol.~7, pp.~394--411, 1990.

\bibitem{Harrison} R.~W.~Harrison ``Phase problem in crystallography,'' \emph{JOSA A}, vol.~10, pp.~1046--1055, 1993.

\bibitem{Hayes} M.~H.~Hayes, J.~S.~Lim, and A.~V.~Oppenheim, ``Signal reconstruction from phase or magnitude,'' \emph{IEEE Trans. Acoust., Speech, Signal Process.}, vol.~28, no.~6, pp.~672--680, 1980.

\bibitem{Bunk} O.~Bunk, A.~Diaz, F.~Pfeiffer, C.~David, B.~Schmitt, D.~K.~Satapathy, and J.~F.~Veen, ``Diffractive imaging for periodic samples: retrieving one-dimensional concentration profiles across microfluidic channels,'' \emph{Acta
Crystallographica Section A: Foundations of Crystallography}, vol.~63, no.~4, pp.~306--314, 2007.

\bibitem{Dainty} J.~C.~Dainty and J.~R.~Fienup, ``Phase retrieval and image reconstruction for astronomy,'' \emph{Image Recovery: Theory and Application, Academic
Press}, pp.~231--275, 1987.

\bibitem{Heinosaari} T.~Heinosaari, L.~Mazzarella, and M.~M.~Wolf, ``Quantum tomography under prior information,'' \emph{Communication in Mathematical Physics}, vol.~318, no.~2, pp.~355--374, 2013.

\bibitem{Baraniuk} M.~L.~Moravec, J.~K.~Romberg, and R.~Baraniuk, ``Compressive phase retrieval,'' in \emph{SPIE Conf. Series}, vol.~6701, 2007.

\bibitem{Candes1} E.~J.~Candes, T.~Strohmer, and V.~Voroninski, ``Phaselift: Exact and stable signal recovery from magnitude measurements via convex programming,''
\emph{Communications on Pure and Applied Mathematics}, vol.~66, no.~8, pp.~1241--1274, 2013.

\bibitem{Candes2} E.~J.~Candes, Y.~C.~Eldar, T.~Strohmer, and V.~Voroninski, ``Phase retrieval via matrix completion,'' \emph{SIAM Journal on Imaging Sciences}, vol.~6, no.~1, pp.~199--225, 2013.

\bibitem{Candes3} E.~J.~Candes, X.~Li, and M.~Soltanolkotabi, ``Phase retrieval from coded diffraction patterns,'' \emph{arXiv preprint arXiv:1310.3240}, 2013.

\bibitem{Mahdi} E.~J.~Candes, X.~Li, and M.~Soltanolkotabi, ``Phase retrieval via Wirtinger flow: theory and algorithms,'' \emph{arXiv preprint arXiv:1407.1065}, 2014.

\bibitem{Candes4}  E.~J.~Candes, J.~Romberg, and T.~Tao, ``Robust uncertainty principles: Exact signal reconstruction from highly incomplete frequency information,'' \emph{IEEE Trans. Inform. Theory}, vol.~52, no.~2, pp.~489--509, 2006.

\bibitem{Rangan} P.~Schniter and S.~Rangan, ``Compressive phase retrieval via generalized approximate message passing,'' \emph{Proceedings of Allerton Conference
on  Communication, Control, and Computing}, 2012.


\bibitem{Rodenburg} J.~M.~Rodenburg, ``Ptychography and related diffractive imaging methods,'' \emph{Advances in Imaging and Electron Physics}, vol.~150, pp.~87--184, 2008.

\bibitem{Hassibi1} K.~Jaganathan, S.~Oymak, and B.~Hassibi, ``Sparse phase retrieval: Convex algorithms and limitations,'' \emph{Proceedings of IEEE International Symposium on Information Theory (ISIT)}, pp.~1022--1026, 2013.

\bibitem{Hassibi2}  K.~Jaganathan, S.~Oymak, and B.~Hassibi, ``Phase retrieval for sparse signals using rank minimization,'' \emph{Proceedings of IEEE International Conference on Acoustics, Speech and Signal Processing}, pp.~3449--3452, 2012.

\bibitem{Sastry} H.~Ohlsson, A.~Yang, R.~Dong, and S.~Sastry, ``Compressive phase retrieval from squared output measurements via semidefinite programming,'' \emph{arXiv preprint, arXiv:1111.6323}, 2011.

\bibitem{Donoho}  D.~Donoho, ``Compressed sensing,'' \emph{IEEE Trans. Inform. Theory}, vol.~52, no.~4, 2006.

\bibitem{Li} X.~Li and V.~Voroninski, ``Sparse signal recovery from quadratic measurements via convex programming,'' \emph{arXiv preprints arXiv:1209.4785}, 2012.

\bibitem{Sanghavi} P.~Netrapalli, P.~Jain, and S.~Sanghavi, ``Phase retrieval using alternating minimization,'' \emph{arXiv preprints arXiv:1306.0160}, 2013.

\bibitem{Alexeev} B.~Alexeev, A.~S.~Bandeira, M.~Fickus, and D.~G.~Mixon, ``Phase retrieval with polarization,'' \emph{arXiv preprint arXiv:1210.7752}, 2012.

\bibitem{Walther} A.~Walther, ``The question of phase retrieval in optics,'' \emph{Optica Acta}, vol.~10, no.~1, pp.~41--49, 1963.

\bibitem{Mohammad} M.~Mirhosseini, O.~S.~Magana-Loaiza, S.~M.~Hashemi~Rafsanjani, R.~W.~Boyd, ``Compressive direct measurement of the quantum wavefunction,'' \emph{arXiv preprint arXiv:1404.2680}, 2014.

\bibitem{Popov} E.~G.~Loewen and E.~Popov, ``Diffraction gratings and applications,'' \emph{CRC Press}, 1997.

\bibitem{Bodmann} B.~G.~Bodmann and N.~Hammen, ``Stable phase retrieval with low-redundancy frames,'' \emph{arXiv preprint arXiv:1302.5487}, 2013.

\bibitem{Tarokh} M.~Akcakaya and V.~Tarokh, ``New conditions for sparse phase retrieval,'' \emph{arXiv preprint arXiv:1310.1351}, 2013.

\bibitem{Waldspurger} I.~Waldspurger, A.~d'Aspremont, and S.~Mallat, ``Phase recovery, maxcut and complex semideﬁnite programming,'' \emph{Mathematical Programming}, pp.~1--35, 2013.

\bibitem{Luby} M.~Luby, ``LT codes,'' \emph{Proc. IEEE Foundations of Computer Science
(FOCS)}, 2002.

\bibitem{Luby2} M.~Luby, M.~Mitzenmacher, M.~A.~Shokrollahi, and D.~Spielman,
``Improved low-density parity check codes using irregular graphs,'' \emph{IEEE
Trans. Info. Theory}, vol.~47, pp.~585--598, 2001.

\bibitem{ER}  Erdos,~P. and Renyi,~A. ``On the evolution of random graphs,'' \emph{Publications of the Mathematical Institute of the Hungarian Academy of Sciences}, vol.~5, pp.~17--61, 1960.

\bibitem{DSP} A.~V.~Oppenheim, R.~W.~Schafer and J.~R.~Buck, ``Discrete-Time Signal 
Processing,'' \emph{Prentice Hall}, 1989. 

\bibitem{RUbook} T.~Richardson and R.~Urbanke, ``Modern Coding Theory,'' \emph{Cambridge
University Press}, 2008.

\bibitem{Wang} Z.~Wang, L.~Millet, M.~Mir, H.~Ding, S.~Unarunotai, J.~Rogers, M.~U.~Gillette, and G.~Popescu, ``Spatial light 
interference microscopy (SLIM),'' \emph{Opt. Express}, vol.~19, no.~2, pp.~1016--1026, 2011. 

\bibitem{Pavani} S.~R.~P.~Pavani and R.~Piestun, ``Three dimensional tracking
of fluorescent microparticles using a photon-limited
double-helix response system,'' \emph{Opt. Express}, vol.~16, pp.~22048--57, 2008.

\end{thebibliography}

